Planning for Multi-Object Manipulation with Graph Neural Network Relational Classifiers

Objects rarely sit in isolation in human environments. As such, we'd like our robots to reason about how multiple objects relate to one another and how those relations may change as the robot interacts with the world. To this end, we propose a novel graph neural network framework for multi-object manipulation to predict how inter-object relations change given robot actions. Our model operates on partial-view point clouds and can reason about multiple objects dynamically interacting during the manipulation. By learning a dynamics model in a learned latent graph embedding space, our model enables multi-step planning to reach target goal relations. We show our model trained purely in simulation transfers well to the real world. Our planner enables the robot to rearrange a variable number of objects with a range of shapes and sizes using both push and pick and place skills.

==> overview_fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
  \begin{center}
    \centering
    \includegraphics[width=\textwidth]{figures/gnn_cover_final.pdf}
    \vspace{-24pt}
  \end{center}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:overview_figure}}~\textbf{Planning using \rdgnn{}:} The robot encodes the segmented scene point cloud into a learned latent state space with graph structure using the encoder \(\Phi\). The robot then plans a sequence of actions using a learned latent dynamics function \(\delta\) to predict relations \(\hat{\rv}\) that match both subgoal \(\gv_1\) and subgoal \(\gv_2\). The robot first plans to push $o_2$ to the right achieving the first subgoal $\gv_1$ then pick-and-place object $o_1$ to be the behind of $o_3$ achieving the second subgoal $\gv_2$ and thus the goal \(\gv = \gv_1 \land \gv_2\). Note relations are defined from the camera's perspective.}
  \vspace{-18pt}
  \medskip}
\makeatother
\shrinka
\maketitle
\shrinka
\thispagestyle{empty}
\pagestyle{empty}


